First Light And Reionisation Epoch Simulations (FLARES) I: Environmental Dependence of High-Redshift Galaxy Evolution

We introduce the First Light And Reionisation Epoch Simulations (FLARES), a suite of zoom simulations using the EAGLE model. We resimulate a range of overdensities during the Epoch of Reionisation (EoR) in order to build composite distribution functions, as well as explore the environmental dependence of galaxy formation and evolution during this critical period of galaxy assembly. The regions are selected from a large $(3.2 \;\mathrm{cGpc})^{3}$ parent volume, based on their overdensity within a sphere of radius $14\,h^{-1}\;\mathrm{cMpc}$. We then resimulate with full hydrodynamics, and employ a novel weighting scheme that allows the construction of composite distribution functions that are representative of the full parent volume. This significantly extends the dynamic range compared to smaller volume periodic simulations. We present an analysis of the galaxy stellar mass function (GSMF), the star formation rate distribution function (SFRF) and the star forming sequence (SFS) predicted by \flares, and compare to a number of observational and model constraints. We also analyse the environmental dependence over an unprecedented range of overdensity. Both the GSMF and the SFRF exhibit a clear double-Schechter form, up to the highest redshifts ($z = 10$). We also find no environmental dependence of the SFS normalisation. The increased dynamic range probed by FLARES will allow us to make predictions for a number of large area surveys that will probe the EoR in coming years, such as WFIRST and Euclid.

==> hmf.tex <==

% \subsection{The Halo Mass Function}

% \begin{figure}
% 	\includegraphics[width=\columnwidth]{images/hmf_all.png}
%     \caption{Redshift evolution of the \flares\ composite (sub)halo mass function, with 1$\sigma$ uncertainties.
%     }
%     \label{fig:hmf_all}
% \end{figure}


\subsection{The Stellar to Halo Mass Relation}



\begin{figure}
	\includegraphics[width=\columnwidth]{images/shmr_all.png}
    \caption{Redshift evolution of the \flares\ composite stellar - halo mass relation.
    Only bins where there are at least 10 galaxies are shown.
    }
    \label{fig:shmr_all}
\end{figure}

